Multi-Physics Model Bias Correction with Data-Driven Reduced Order Modelling Techniques: Application to Nuclear Case Studies

Nowadays, interest in combining mathematical knowledge about phenomena and data from the physical system is growing. Past research was devoted to developing so-called high-fidelity models, intending to make them able to catch most of the physical phenomena occurring in the system. Nevertheless, models will always be affected by uncertainties related, for example, to the parameters and inevitably limited by the underlying simplifying hypotheses on, for example, geometry and mathematical equations; thus, in a way, there exists an upper threshold of model performance. Now, research in many engineering sectors also focuses on the so-called data-driven modelling, which aims at extracting information from available data to combine it with the mathematical model. Focusing on the nuclear field, interest in this approach is also related to the Multi-Physics modelling of nuclear reactors. Due to the multiple physics involved and their mutual and complex interactions, developing accurate and stable models both from the physical and numerical point of view remains a challenging task despite the advancements in computational hardware and software, and combining the available mathematical model with data can further improve the performance and the accuracy of the former. This work investigates this aspect by applying two Data-Driven Reduced Order Modelling (DDROM) techniques, the Generalised Empirical Interpolation Method and the Parametrised-Background Data-Weak formulation, to literature benchmark nuclear case studies. The main goal of this work is to assess the possibility of using data to perform model bias correction, that is, verifying the reliability of DDROM approaches in improving the model performance and accuracy through the information provided by the data. The obtained numerical results are promising, foreseeing further investigation of the DDROM approach to nuclear industrial cases.

==> schemes/DA_ROM.tex <==
\begin{tikzpicture}
		
		%% Input layer
		\node[circle,draw=black,minimum size =4, fill=blue] (input-1) at (0,0){};
		\foreach \i in {1,...,9}
		{
			\pgfmathtruncatemacro{\x}{\i + 1};
			\node[circle,draw=black,minimum size =4, fill=blue, below=0.1cm of input-\i] (input-\x) {};
		}
		
		%% Reduced layer
		\node[circle,draw=black,minimum size =4, fill=greenPolimi!50, right=3cm of input-4] (reduced-1) {};
		\foreach \i in {1,...,3}
		{
			\pgfmathtruncatemacro{\x}{\i + 1};
			\node[circle,draw=black,minimum size =4, fill=greenPolimi!50, below=0.1cm of reduced-\i] (reduced-\x) {};
		}
		
		%% Data-enhanced layer
		\foreach \i in {1,...,4}
		{
		\node[circle,draw=black,minimum size =4, fill=red, right=4cm of reduced-\i] (dataEnhanced-\i) {};
		}
		
		%% Output layer
		\node[circle,draw=black,minimum size =4, fill=blue, right=11cm of input-1] (output-1) {};
		\foreach \i in {1,...,9}
		{
			\pgfmathtruncatemacro{\x}{\i + 1};
			\node[circle,draw=black,minimum size =4, fill=blue, below=0.1cm of output-\i] (output-\x) {};
		}
		
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		
		\node[draw,black,line width=0.75pt, inner sep=1mm,fit=
		(input-1)
		(input-2)
		(input-3)
		(input-4)
		(input-5)
		(input-6)
		(input-7)
		(input-8)
		(input-9)
		(input-10)
		] {};
		
		\node[draw,black,line width=0.75pt, inner sep=1mm,fit=
		(reduced-1)
		(reduced-2)
		(reduced-3)
		(reduced-4)
		] {};
		
		\node[draw,black,line width=0.75pt, inner sep=1mm,fit=
		(dataEnhanced-1)
		(dataEnhanced-2)
		(dataEnhanced-3)
		(dataEnhanced-4)
		] {};
		
		
		\node[draw,black,line width=0.75pt, inner sep=1mm,fit=
		(output-1)
		(output-2)
		(output-3)
		(output-4)
		(output-5)
		(output-6)
		(output-7)
		(output-8)
		(output-9)
		(output-10)
		] {};
		
		
		\draw[-, line width = 1pt] (0.35,0.25) -- (3.,-1.1);
		\draw[-, line width = 1pt] (0.35,-4.25) -- (3.,-2.9);
		
		
		\draw[-, line width = 1pt] (3.625,-1.1) -- (7.42,-1.1);
		\draw[-, line width = 1pt] (3.625,-2.9) -- (7.425,-2.9);
		\node[text centered,  text width=3.5cm, minimum height = 1.75cm] (DAprocess) at (5.515, -2) {Data Assimilation};
		
		\draw[-, line width = 1pt] (8.05,-1.1) -- (11.,0.25);
		\draw[-, line width = 1pt] (8.05,-2.9) -- (11.,-4.25);
		
		\node[text centered,  text width=2cm, above right= 0.25cm and -1.2cm of input-1] (FOM-1) {Full Order $\mathbf{u}\in\mathbb{R}^{\mathcal{N}_h}$};
		\node[text centered, text width=2.75cm, above right= 0.25cm and -1.5cm of output-1] (FOM-2) {State Estimation \\ $\mathbf{u}^\star\in\mathbb{R}^{\mathcal{N}_h}$};
		\node[text centered, text width=3.5cm, above right= 0.25cm and -1.85cm of reduced-1] (ROM) {Reduced \\Background \\ $\boldsymbol{\alpha}\in\mathbb{R}^N$};
		\node[text centered, text width=3.5cm, above right= 0.25cm and -2cm of dataEnhanced-1] (DA-ROM) {Updated \\Knowledge \\ $\boldsymbol{\alpha}^\star\in\mathbb{R}^{N+M}$};
		
		
		\node[text centered,  text width=2cm,below right= -0.35cm and 0.25cm of input-5] (encoding-proc) {Dimensionality Reduction\\
		$\mathcal{N}_h>>N$};
		\node[text centered,  text width=2.5cm,below left= -0.35 and 0.25cm of output-5] (decoding-proc) {State \\Estimation\\
		$N+M<<\mathcal{N}_h$};
		
		
		\node[draw,fill = green2!40, text centered,  text width=2.5cm, below = 0.8cm of DAprocess] (measure) {Measurements\\ $\mathbf{y}\in\mathbb{R}^M$};
		
		
		\draw[->, line width = 2pt] (measure.north) -- (DAprocess.south);
		
		\draw[->, draw = green2, line width = 1pt] (3.33, -3) |- (measure.west) ;
		
		\node[text centered,  text width=2cm, left= 0.4cm of measure] (measure-place) {\color{green2}Sensors Placement};
		
		
		\draw[-, line width = 3pt, draw = green2!60] (0, -5) -- (5.5, -5)
		node[midway,below]{\color{green2!80}Offline/Training Phase};
		\draw[-, line width = 3pt, draw = red] (5.5, -5) -- (11.35, -5)
		node[midway,below]{\color{red}Online Phase};
		\draw[-, line width = 3pt] (0, -5.25) -- (0, -4.75);
		\draw[-, line width = 3pt] (5.5, -5.25) -- (5.5, -4.75);
		\draw[-, line width = 3pt] (11.35, -5.25) -- (11.35, -4.75);
		
\end{tikzpicture}
